Sensory Glove-Based Surgical Robot User Interface

Robotic surgery has reached a high level of maturity and has become an integral part of standard surgical care. However, existing surgeon consoles are bulky, take up valuable space in the operating room, make surgical team coordination challenging, and their proprietary nature makes it difficult to take advantage of recent technological advances, especially in virtual and augmented reality. One potential area for further improvement is the integration of modern sensory gloves into robotic platforms, allowing surgeons to control robotic arms intuitively with their hand movements. We propose one such system that combines an HTC Vive tracker, a Manus Meta Prime 3 XR sensory glove, and SCOPEYE wireless smart glasses. The system controls one arm of a da Vinci surgical robot. In addition to moving the arm, the surgeon can use fingers to control the end-effector of the surgical instrument. Hand gestures are used to implement clutching and similar functions. In particular, we introduce clutching of the instrument orientation, a functionality unavailable in the da Vinci system. The vibrotactile elements of the glove are used to provide feedback to the user when gesture commands are invoked. A qualitative and quantitative evaluation has been conducted that compares the current device with the dVRK console. The system is shown to have excellent tracking accuracy, and the new interface allows surgeons to perform common surgical training tasks with minimal practice efficiently.

==> figures/confusion_prediction.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}{0.49\columnwidth}
        \includegraphics[trim={0.5cm 1cm 1.5cm 0cm}, clip, width=\columnwidth]{figures/confusion_matrices/confusion_matrix_nn.pdf}
        \caption{MLP}
        \label{fig:cm_mlp}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\columnwidth}
        \includegraphics[trim={0.5cm 1cm 1.5cm 0cm}, clip, width=\columnwidth]{figures/confusion_matrices/confusion_matrix_lgbm.pdf}
        \caption{L-GBM}
        \label{fig:cm_lgbm}
    \end{subfigure}
    
    \begin{subfigure}{0.49\columnwidth}
        \includegraphics[trim={0.5cm 1cm 1.5cm 0cm}, clip, width=\columnwidth]{figures/confusion_matrices/confusion_matrix_rf.pdf}
        \caption{Random Forest}
        \label{fig:cm_rf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\columnwidth}
        \includegraphics[trim={0.5cm 1cm 1.5cm 0cm}, clip, width=\columnwidth]{figures/confusion_matrices/confusion_matrix_hist.pdf}
        \caption{HGBT}
        \label{fig:cm_hgbt}
    \end{subfigure}
    \caption{Confusion matrices for gesture recognition models.}
    \label{fig:confusion}
    \vspace{-3mm}
\end{figure}


==> figures/gesture_prediction_figures.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.15\textwidth}
        \includegraphics[width=\textwidth]{figures/gestures/clutch_prediction.pdf}
        \caption{}
        \label{fig:clutch_prediction}
    \end{subfigure}
    \begin{subfigure}[b]{0.15\textwidth}
        \includegraphics[width=\textwidth]{figures/gestures/none_prediction.pdf}
        \caption{}
        \label{fig:none_prediction}
    \end{subfigure}
    \begin{subfigure}[b]{0.15\textwidth}
        \includegraphics[width=\textwidth]{figures/gestures/thumbup_prediction.pdf}
        \caption{}
        \label{fig:thumbup_prediction}
    \end{subfigure}
    \begin{subfigure}[b]{0.15\textwidth}
        \includegraphics[width=\textwidth]{figures/gestures/rf_prediction.pdf}
        \caption{}
        \label{fig:thumbup_prediction}
    \end{subfigure}
    \begin{subfigure}[b]{0.15\textwidth}
        \includegraphics[width=\textwidth]{figures/gestures/pinky_prediction.pdf}
        \caption{}
        \label{fig:thumbup_prediction}
    \end{subfigure}
    \caption{3D Positions of Landmarks received by the model and its outputted predictions }
    \label{fig:predictions}
\end{figure}

==> figures/glove_psm_tf/glove_psm_distance.tex <==
\begin{figure}[t!]
\centering
%\includesvg[width=\columnwidth]{glove_psm_dist}
\includegraphics[width=\columnwidth]{glove_psm_dist}
\caption{Translational and orientational distance between the glove and the PSM: the left figure depicts the Euclidean distance, while the right one details the orientation difference, quantified with rotation matrices (in the hand workspace).}

%(d) focuses on a portion of the motion in translation when the clutch was disengaged, demonstrating the alignment within the 3D space.

\label{fig:glove_psm_dist}
\vspace{-3mm}
\end{figure}

==> figures/test.tex <==
\begin{figure*}
    \begin{minipage}[t]{0.45\textwidth}
        \centering
        \includesvg[width=\linewidth]{figures/glove_psm_tf/glove_psm_P}
        \caption{Translation}
        \label{fig:glove_psm_P}
    \end{minipage}\hfill
    \begin{minipage}[t]{0.45\textwidth}
        \centering
        \includesvg[width=\linewidth]{figures/glove_psm_tf/glove_psm_R}
        \caption{Orientation}
        \label{fig:glove_psm_R}
    \end{minipage}
    
    \begin{minipage}[t]{0.45\textwidth}
        \centering
        \includesvg[width=\linewidth]{figures/glove_psm_tf/glove_psm_jaw}
        \caption{Jaw Movements}
        \label{fig:glove_psm_jaw}
    \end{minipage}\hfill
    \begin{minipage}[t]{0.45\textwidth}
        \centering
        \includegraphics[trim={1cm 0cm 1cm 0cm}, clip, width=\linewidth]{figures/glove_psm_tf/glove_psm_delay.pdf}
        \caption{}
        \label{fig:glove_psm_dtw}
    \end{minipage}
    
    \begin{minipage}[t]{0.45\textwidth}
        \centering
        \includesvg[width=\linewidth]{figures/glove_psm_tf/glove_psm_dist}
        \caption{}
        \label{fig:glove_psm_dist}
    \end{minipage}\hfill
    \begin{minipage}[t]{0.45\textwidth}
        \centering
        \input{tables/exercise_res}
        \captionof{table}{Exercise Results}
        \label{tab:ex_res}
    \end{minipage}
    
    \caption{(a-c) A sample recording of motion between the glove and the PSM. The segments highlighted in purple indicate periods when the clutch mechanism was engaged. (a) displays the translation of the glove and PSM while (b) shows the orientation of the glove and PSM respectively. (c) compares the distance of the thumb and index finger on the glove with the jaw angle of the PSM. (d) and (e) detail the x-axis translation of the glove and the PSM tip in Fig.~\ref{fig:glove_psm_P}. The initial plot illustrates a delay in the robot's execution of the glove's movements. To address this, the delay between the signals was measured based on the peaks, and the aligned signals were shown on the bottom. (e) Translational and orientational distance between the glove and the PSM: the left figure depicts the Euclidean distance, while the right one details the orientation difference, quantified using quaternions (in the hand workspace).}
    \label{fig:glove_psm_T}
\end{figure*}


==> sections/clutch_old.tex <==



\subsubsection{Clutch in rotation}\hfill 

\textbf{Clutching}: When the clutch is engaged,  we save the rotation of the tracker denoted as $R$ and we keep it constant (renamed $R_{cn}$). This will activate the vibrotactile feedback of the glove.
    
\textbf{High-to-low transition (edge) of the Clutch}: The last rotation of the tracker denoted as $R_c$, is saved.
    
\textbf{Not Clutching}: When the clutch is disengaged, $R_{rel}$ is determined as the inverse of $R_c$ (last rotation at the end of the clutch) times $R_{cn}$ (last rotation right before clutching).
    \[
    R_{rel}=R_c^{-1}R_{cn}
    \]
Therefore the resultant quantity, $R_r$, is obtained by multiplying $R_{cn}$ by $R_{rel}$. This will be used as input for the controller.
    \[R_r=R_mR_{rel}=R_mR_c^{-1}R_{rel}\]
It is important to note that to allow faster computation we worked with normalized quaternions as its inverse is simply its conjugate.

\begin{algorithm}[t]
\caption{Clutch}
\label{alg:clutch}
\SetAlgoNlRelativeSize{0}
\SetAlgoNlRelativeSize{-1}
\SetAlgoNlRelativeSize{-2}
\SetAlgoNoEnd

\If{clutch\_engaged}{
    
    $R \gets R_{cn}$\;
    $p \ \text{unchanged}$\;
    $p_b\gets p_t$\;
}
\ElseIf{High-to-low transition  of the Clutch}{
    $p_{bt} \gets p_t$\;
    save $R_c$\;
}
\Else{
    $R_{\text{rel}} \gets \text{inverse}(R_c)  R_{\text{cn}}$\;
    $R_r \gets R_{cn}  R_{\text{rel}}$\;
    $p \gets p_t - p_{bt} - p_c$\;
}
\end{algorithm}

\subsubsection{Clutch in translation }\hfill

\textbf{Clutch}: we translate the Tracker Base ($p_b$) for the translation between the Base Station and the Tracker $p_t$, applying the last saved translation before clutching as the current input position $p$, and saving it as an additional offset $p_c$. This activates the vibrotactile feedback of the glove.

\textbf{High-to-low transition (edge) of the Clutch}: we save the last translation between the Base Station and the Tracker as $p_{bt}$.

\textbf{NOT Clutch}: we translate the tracker (input) t.r. of the Tracker Base of the measured distance between the Base Station and the Tracker minus the two saved offsets:
\[
p=p_t-p_c-p_{bt}
\]
The operation of the clutch is described on Algorithm~\ref{alg:clutch}.


==> tables/gesture_dataset.tex <==
\begin{table}[htbp]
\centering
\begin{tabular}{c|c|c|c}
\hline \hline
\textbf{Gesture} & \textbf{Clutch} & \textbf{Ring}& \textbf{None} \\
\hline
\textbf{Quantity} & 15557 & 17036 & 178217\\
\hline \hline
\end{tabular}
\caption{Quantities of each class for gestures.}
\label{tab:gesture_quantities}
\end{table}

